Impacts of Students Academic Performance Trajectories on Final Academic Success

Many studies in the field of education analytics have identified student grade point averages (GPA) as an important indicator and predictor of students' final academic outcomes (graduate or halt). And while semester-to-semester fluctuations in GPA are considered normal, significant changes in academic performance may warrant more thorough investigation and consideration, particularly with regards to final academic outcomes. However, such an approach is challenging due to the difficulties of representing complex academic trajectories over an academic career. In this study, we apply a Hidden Markov Model (HMM) to provide a standard and intuitive classification over students' academic-performance levels, which leads to a compact representation of academic-performance trajectories. Next, we explore the relationship between different academic-performance trajectories and their correspondence to final academic success. Based on student transcript data from University of Central Florida, our proposed HMM is trained using sequences of students' course grades for each semester. Through the HMM, our analysis follows the expected finding that higher academic performance levels correlate with lower halt rates. However, in this paper, we identify that there exist many scenarios in which both improving or worsening academic-performance trajectories actually correlate to higher graduation rates. This counter-intuitive finding is made possible through the proposed and developed HMM model.

==> application.tex <==
\section{Applying HMM to student data}
  



==> oldFiles/conclusion.tex <==
In this paper, we analyzed students' academic-performance trajectories at \censor{University of Central Florida} and examined their final academic outcomes in terms of halt rates. Unlike traditional statistical methodologies, our proposed approach is able to provide a standard point of reference for comparing students GPA performance both across their enrolled semesters and across all students. Our proposed HMM model takes the sequence of course grades over multiple semesters and returns the sequence of estimated academic-performance levels. The estimated HMM parameters illustrate that while W grades are not involved in computing students' GPA, there is significant relationship between students' academic-performance level and withdrawing from courses. Also, by tracking students transition between four main academic-performance levels, we observed that a significant portion of students (43.30\%), acquire a combination of academic-performance levels during their education, a timely learning of which can provide invaluable directions to universities policy makers.  Furthermore, analyzing halt rate for students with a consistent academic performance levels suggested that students who constantly maintain a low academic-performance level are more likely to leave school without a degree. For students with a change in their academic-performance level it was shown that switching from any academic-performance levels to level 1 increases the halt rate substantially. However for some academic-performance trajectories with switching from a high academic performance level to a lower, does not necessarily result in a higher halt rate. The investigation of the underlying reason for such observation is left as a good avenue for future qualitative research. 

==> oldFiles/introduction.tex <==
Does an improvement in 

That is to say, a student that started with a low GPA and improved their grades with time would be equivalent to a student that maintained the same GPA over their academic career. 

To prioritize at-risk students, it is important to identify students who have demonstrated a more significant downward pattern in their GPA trajectory compared to their peers. This, however, is not possible with the traditional statistical methods as they can only detect notable status changes across one student's GPA pathway. For universities to be able to prioritize at-risk students, they would rather need a holistic and standard point of reference for making department-wide or school-wide comparisons.


The HMM parameters are learnt based on real-world academic transcripts for first-time-in-college (FTIC) students. to provide a standard classification of students' semester academic-performance into four levels. This methodology provides a valuable asses to university principals to compare a student's performance in a semester based on both his previous performance and performance of his peers across the university, and therefore better prioritize students for receiving financial and academic supports. We also investigate the enrollment halt rate for students with different academic-performance level trajectories to provide more insights into the relationship between academic-performance level and drop out rate. 

==> oldFiles/methodology.tex <==
Each Hidden Markov Model corresponds with a set of state $Q=\{q_1,q_2,\hdots,q_N\}$, with $N$ representing number of different states. Unlike any other types of Markov models in which the states are observable, in HMMs, states are hidden; that is, it is unknown at which states the system dwells at any particular moment. The goal of HMM is then to estimate a sequence of the hidden states. The state sequences can be of different lengths, $T$, and are estimated using a sequence of observations, $O=o_1,o_2,\hdots,o_T$, that are generated from the states. Each HMM has the following three parameters: (1) $A=[a_{i,j}]\in\mathcal{R}^{NxN}$ which is a transition matrix that shows the probabilities by which system moves between the hidden states (2) $B=b_i(o_t)$ an emission matrix which demonstrate the probability of generating observation $o_t$ when the system is in state $q_i$, and (3) $\pi_0$, the probability distribution for the system being at a particular state initially.

The first step to build an HMM, known as the \textsc{learning step}, is to estimate the optimal values for the parameters $\lambda=(A, B,\pi_0)$. We use the Baum-Welch algorithm, a kind of expectation-maximization algorithm, to estimate the optimal parameters $\lambda^*$. This algorithm takes initial guesses for each of the parameters and iteratively improves the estimations of the parameters by computing the likelihood of any sequence of observation given $\lambda$. After obtaining the optimal $\lambda^*$, the next step is to predict the sequence of hidden states for a given observation sequence. This step, known as \textsc{decoding step} uses the Viterbi algorithm, which takes observation sequences and $\lambda^*$ as input and returns estimated hidden states as the output.    

==> oldFiles/problemstatement.tex <==
\section{Problem Statement} \label{sec:problem_statment}
In this paper, we analyse students' GPA trajectories based on the grades of the courses they take each semester. Students from starting their education until finishing it, may have different academic performance trajectories. Some of these trajectories have results in graduation with high degree GPA, some other low degree GPA, and some other may have results in halting. So it is important to monitor students' performance, specifically for students who are at the risk of leaving school without degree. 

Previously, many research have conducted to predict future students' academic performance based on their background. Most of these studies have used students' academic and demographic  information until a certain semester to predict academic performance for the rest of the semesters \cite{olani2009predicting,marbouti2016models,huang2013predicting}. An issue that these studies have been faced is to determine the optimal time to apply the prediction models during semester. In other words, making prediction too early may not has high accuracy, however late prediction gives students little time to improve their academic performance. In this study, we apply Hidden Markov Model to classify students based on their GPA level and then investigate the relationship between different GPA trajectories and academic success. Since this predicts students performance dynamically over time, there is no need to find the optimal time for prediction.

For each student in each semester, we consider a vector with five elements, in which the first, second, and third elements are integers showing the number of courses with the A, B, and C grade, respectively. Fourth and fifth elements are binary variables, demonstrating if the student has any courses with the D/F and W grade, respectively. The created hidden Markov model, takes a sequence of observations (vectors) for each student and returns a sequence of estimated hidden states (GPA Level). In order to decrease dimensionality of the problem, for the first, second the third elements in the grade number vector, we assign 3 if students have 3 or more courses with the grade of A, B, and C respectively. Therefore, the first to third elements could get any values from 0 to 3, and the fourth and fifth elements are binary (0 and 1). 

After initiating vectors for each student in each semester, we convert each distinct vector into a single integer number and consider it as an HMM observation. Going through students' transcripts, there are 216 distinct different combinations of vector grades, therefore, the HMM observation could be any number from 0 to 215. The output of the model is the estimated GPA level that is an integer number between 1 to 4. Level 1 and 4 corresponds to the lowest and highest academic performance respectively. Given the estimated GPA level for each student in each semester as an standard reference, we can track students' academic performances during their academic career. As mentioned earlier this GPA trajectory tracking helps university policymakers to inform students who are at the risk of halting their studies and prioritize then for receiving supports. \tabref{tab:HMM_input_output} presents the input and output of HMM for some arbitrary students. 

\begin{table}
\centering
\caption{Example students' grade vector sequence and corresponding estimated GPA leve sequence}
\begin{tabular}{|c|c|c|} \hline
Student &Grade vector Seq.& GPA level Seq.\\ \hline
1&00011,10100,00211,00011 & 1,1,1,1\\ \hline
2&11110,11200,21001,13000 & 2,2,2,2\\ \hline
3&22000,32000,30100 & 3,3,3\\ \hline
4&30000,31000,30000 & 4,4,4 \\ \hline
5&30000,30000,00010,00010 & 4,4,1,1\\
\hline\end{tabular}
\label{tab:HMM_input_output}
\end{table}

Based on \tabref{tab:HMM_input_output}, student number 1 has enrolled in four semesters at UCF so far as he has four grade vector recorded in his history. In the first semester, he has no courses with A, B, or C grade as the first three digits are all zero. The forth and fifth digit in the grade vector shows that this student has grade DF and W in his first semester. His grade vector for rest of the semesters are explained the same manner.  The estimated GPA level for this student in all enrolled semesters is 1. As we see in the table, while students number 1 to 4 have a consistent GPA level during their academic careers, GPA level for student number 5 has changed from 4 to 1 in his third semester.
 


